Phase Transitions in Ising models: the Semi-infinite with decaying field and the Random Field Long-range

In this thesis, we present results on phase transition for two models: the semi-infinite Ising model with a decaying field, and the long-range Ising model with a random field. We study the semi-infinite Ising model with an external field $h_i = \lambda |i_d|^{-\delta}$, $\lambda$ is the wall influence, and $\delta>0$. This external field decays as it gets further away from the wall. We are able to show that when $\delta>1$ and $\beta > \beta_c(d)$, there exists a critical value $0< \lambda_c:=\lambda_c(\delta,\beta)$ such that, for $\lambda<\lambda_c$ there is phase transition and for $\lambda>\lambda_c$ we have uniqueness of the Gibbs state. In addition, when $\delta<1$ we have only one Gibbs state for any positive $\beta$ and $\lambda$. For the model with a random field, we extend the recent argument by Ding and Zhuang from nearest-neighbor to long-range interactions and prove the phase transition in the class of ferromagnetic random field Ising models. Our proof combines a generalization of Fr\"ohlich-Spencer contours to the multidimensional setting proposed by Affonso, Bissacot, Endo and Handa, with the coarse-graining procedure introduced by Fisher, Fr\"ohlich, and Spencer. Our result shows that the Ding-Zhuang strategy is also useful for interactions $J_{xy}=|x-y|^{- \alpha}$ when $\alpha > d$ in dimension $d\geq 3$ if we have a suitable system of contours, yielding an alternative proof that does not use the Renormalization Group Method (RGM), since Bricmont and Kupiainen claimed that the RGM should also work on this generality. We can consider i.i.d. random fields with Gaussian or Bernoulli distributions.

==> Capitulo_2/2.1_Phase_transition_with_non-homogeneous_external_field.tex <==
Every sequence $\mathrm{h}=(\mathrm{h}_k)_{k=0}^\infty$ induces an external field $\bm{\rmh}$ given by $\bm{\rmh}_i = \rmh_{i_d}$, for all $i\in\H+$. In this section, we consider the semi-infinite model with external field $\bm{\rmh}$ with the sequence $\rmh$ being summable. 
We prove a proposition similar to Proposition \ref{PF.1} and then we compare $\tau_w(J,\lambda,\bm{\rmh})$ and $\tau_w(J,\lambda,0)$. By doing so, we are able to prove the theorem

\begin{theorem}
Let $J>0$, $\lambda\geq 0$ and $\bm{\rmh}$ be an external field induced by a summable sequence $\mathrm{h}=(\mathrm{h}_k)_{k=0}^\infty$, i.e.,

\begin{equation*}
    \sum_{k=0}^\infty \mid \mathrm{h}_k \mid < \infty.
\end{equation*}
Then, if 8$\sum_{k=0}^\infty \mid \mathrm{h}_k \mid < \tau_w(J, \lambda, 0)$ and $\lambda< \lambda_c$, there is partial wetting. 
\end{theorem}
This theorem follows from the next two results. 

\begin{proposition}\label{compare.st.and.integral}
Let $J>0$, $\lambda\geq 0$ and $\bm{\rmh}$ be an external field induced by a summable sequence $\mathrm{h}=(\mathrm{h}_k)_{k=0}^\infty$. Then
\begin{equation}
    \mid \tau_w(J,\lambda, \bm{\rmh}) - \int_0^\lambda \langle \sigma_0 \rangle^{+, \bm{\rmh}}_{J,s} - \langle \sigma_0 \rangle^{-,\bm{\rmh}}_{J,s} ds\mid \leq 4\sum_{k=0}^\infty \mid \mathrm{h}_k \mid. 
\end{equation}
\end{proposition}

\begin{proof}
As $J$ is a fixed parameter, we are omitting if from the notation. We start by writing 

\begin{equation}\label{tauw.limit}
    \tau_w(J,\lambda, \bm{\rmh}) = \lim_{n \to \infty} -\frac{1}{|\mathcal{W}_n|}\ln\left[ \frac{\mathcal{Z}^{-}_{n; \lambda,\bm{h}}}{\mathcal{Z}^{+}_{n; \lambda,\bm{h}}} \right] - \frac{1}{2|\mathcal{W}_n|}\ln\left[ \frac{Q^{+}_{\Delta_n; \bm{\rmh}}}{Q^{-}_{\Delta_n; \bm{\rmh}}} \right].
\end{equation}

For the first term in (\ref{tauw.limit}) we compute
\begin{align*}
    \frac{d}{d \lambda} \ln\left[ \frac{\mathcal{Z}^{-}_{n; \lambda,\bm{h}}}{\mathcal{Z}^{+}_{n; \lambda,\bm{h}}} \right] = \sum_{i\in \mathcal{W}_n}  \langle \sigma_i \rangle^{-}_{n; \lambda, \bm{\rmh}} -  \langle \sigma_i \rangle^{+}_{n; \lambda, \bm{\rmh}}
\end{align*}
and get
\begin{align*}
    -\frac{1}{|\mathcal{W}_n|}\ln\left[ \frac{\mathcal{Z}^{-}_{n; \lambda,\bm{h}}}{\mathcal{Z}^{+}_{n; \lambda,\bm{h}}} \right] &= -\frac{1}{|\mathcal{W}_n|} \int_0^{\lambda} \frac{d}{d s} \ln\left[ \frac{\mathcal{Z}^{-}_{n; s,\bm{h}}}{\mathcal{Z}^{+}_{n; s,\bm{h}}} \right] ds - \frac{1}{|\mathcal{W}_n|} \ln\left[ \frac{\mathcal{Z}^{-}_{n; 0,\bm{h}}}{\mathcal{Z}^{+}_{n; 0,\bm{h}}} \right] \\
        &= \frac{1}{|\mathcal{W}_n|} \sum_{i\in \mathcal{W}_n} \int_0^\lambda   \langle \sigma_i \rangle^{+}_{n; s, \bm{\rmh}} -  \langle \sigma_i \rangle^{-}_{n; s, \bm{\rmh}} ds - \frac{1}{|\mathcal{W}_n|} \ln\left[ \frac{\mathcal{Z}^{-}_{n; 0,\bm{h}}}{\mathcal{Z}^{+}_{n; 0,\bm{h}}} \right].
\end{align*}

By the same argument used in the proof of Proposition \ref{PF.1},
\begin{equation*}
    \lim_{n\to\infty} \frac{1}{|\mathcal{W}_n|} \sum_{i\in \mathcal{W}_n} \int_0^\lambda   \langle \sigma_i \rangle^{+}_{n; s, \bm{\rmh}} -  \langle \sigma_i \rangle^{-}_{n; s, \bm{\rmh}} ds = \int_0^\lambda   \langle \sigma_0 \rangle^{+}_{ s, \bm{\rmh}} -  \langle \sigma_0 \rangle^{-}_{s, \bm{\rmh}} ds,
\end{equation*}
hence \eqref{tauw.limit} yields

\begin{equation}\label{Eq: tau_omega_with_field_2}
    \tau_w(J,\lambda, \bm{\rmh}) = \int_0^\lambda   \langle \sigma_0 \rangle^{+}_{s, \bm{\rmh}} -  \langle \sigma_0 \rangle^{-}_{s, \bm{\rmh}} ds + \tau_w(\bm{J}, 0, \bm{\rmh}).
\end{equation}

The proposition follows by bounding the two terms of 
\begin{equation}
    \tau_w(J, 0, \bm{\rmh}) = \lim_{n \to \infty} -\frac{1}{|\mathcal{W}_n|}\ln\left[ \frac{\mathcal{Z}^{-}_{n; 0,\bm{h}}}{\mathcal{Z}^{+}_{n; 0,\bm{h}}} \right] - \frac{1}{2|\mathcal{W}_n|}\ln\left[ \frac{Q^{+}_{\Delta_n; \bm{\rmh}}}{Q^{-}_{\Delta_n; \bm{\rmh}}} \right].
\end{equation}

When $\h\equiv 0$, $Q^{+}_{\Delta_n; 0} = Q^{-}_{\Delta_n; 0}$ by spin flipping, but this not true when the external field is non zero. However, we can bound

\begin{align}\label{bound.in.Q+}
     Q^{+}_{\Delta_n; \bm{\rmh}} &\leq \sum_{\omega \in \Omega^+_{\Delta_n}} \exp{\{ \sum_{\substack{ i \sim j \\ \{ i,j \}\cap \Delta_n \neq \emptyset}} J\sigma_i\sigma_j + \sum_{i\in\Delta_n} \mid h_i\mid \}}\\
                                    &= \exp{\{\sum_{i\in\Delta_n} \mid h_i\mid \}} Q^+_{\Delta_n; 0} = \exp{\{2(2n+1)^{d-1} \sum_{k=0}^{\lfloor n^\alpha \rfloor} \mid \mathrm{h}_k\mid \} }Q^+_{\Delta_n; 0}
\end{align}
       
       and, similarly,
       
\begin{equation}\label{bound.in.Q-}
    Q^{-}_{\Delta_n; \bm{\rmh}} \geq  \exp{\{-2(2n+1)^{d-1} \sum_{k=0}^{\lfloor n^\alpha \rfloor} \mid \mathrm{h}_k\mid \} }Q^-_{\Delta_n; 0}.
\end{equation}       
       
Hence
\begin{align*}
          - \frac{1}{2|\mathcal{W}_n|}\ln\left[ \frac{Q^{+}_{\Delta_n; \bm{\rmh}}}{Q^{-}_{\Delta_n; \bm{\rmh}}} \right] &\geq -\frac{1}{2|\mathcal{W}_n|}\ln\left[ \exp{\{4(2n+1)^{d-1} \sum_{k=0}^{\lfloor n^\alpha \rfloor} \mid \mathrm{h}_k \mid\}} \frac{Q^{+}_{\Delta_n; 0}}{Q^{-}_{\Delta_n; 0}} \right] \\
          &= -2(\frac{2n +1}{2n})^{d-1} \sum_{k=0}^{\lfloor n^\alpha \rfloor} \mid \mathrm{h}_k\mid.
\end{align*}

Alternating the bounds in (\ref{bound.in.Q+}) and (\ref{bound.in.Q-}) we get a similar upper bound, thus

\begin{equation}\label{bound.on,Q+/Q-}
      \mid \frac{1}{2|\mathcal{W}_n|}\ln\left[ \frac{Q^{+}_{\Delta_n; \bm{\rmh}}}{Q^{-}_{\Delta_n; \bm{\rmh}}} \right] \mid \leq 2(\frac{2n +1}{2n})^{d-1} \sum_{k=0}^{\lfloor n^\alpha \rfloor} \mid \mathrm{h}_k\mid.
\end{equation}

Again, for the second term we have that $\mathcal{Z}^{+}_{n; 0,0}=\mathcal{Z}^{-}_{n; 0,0}$ and then we can use the same bounds as in (\ref{bound.in.Q+}) and (\ref{bound.in.Q-}) to get 

\begin{equation*}
    \mid \ln\left[ \frac{\mathcal{Z}^{-}_{n; 0,\bm{h}}}{\mathcal{Z}^{+}_{n; 0,\bm{h}}} \right] \mid \leq 2(2n+1)^{d-1} \sum_{k=0}^{\lfloor n^\alpha\rfloor} \mid \mathrm{h}_k \mid.
\end{equation*}

 Finally,
 \begin{align*}
     \mid \tau_w(J,\lambda, \bm{\rmh}) - \int_0^\lambda \langle \sigma_0 \rangle^{+, \bm{\rmh}}_{J,s} - \langle \sigma_0 \rangle^{-,\bm{h}}_{J,s} ds\mid &\leq \lim_{n\to\infty} \frac{1}{|\mathcal{W}_n|} \mid \frac{1}{2}\ln\left[ \frac{Q^{+}_{\Delta_n; \bm{\rmh}}}{Q^{-}_{\Delta_n; \bm{\rmh}}} \right] +  \ln\left[ \frac{\mathcal{Z}^{-}_{n; 0,\bm{h}}}{\mathcal{Z}^{+}_{n; 0,\bm{h}}} \right] \mid \\
        &= 4\sum_{k=0}^{\infty} \mid \mathrm{h}_k \mid.
 \end{align*}
\end{proof}

Now we proceed to compare $\tau_w$ for the cases with a without the external field.

\begin{lemma}\label{compare.surface.tension}
For $J>0$, $\lambda\geq 0$ and $\bm{h}=(h_k)_{k=0}^\infty$ summable,

\begin{equation}\label{t-tw}
    \mid \tau_w(J,\lambda, \bm{\rmh}) - \tau_w(J,\lambda, 0) \mid\leq 4\sum_{k=0}^\infty \mid \mathrm{h}_i \mid. 
\end{equation}
\end{lemma}

\begin{proof}

 The equation (\ref{excahnge.for.mp}) gives us 
 \begin{equation}
     \tau_w(J,\lambda,\bm{h})=  \lim_{n \to \infty} -\frac{1}{|\mathcal{W}_n|}\ln\left[ \frac{\mathcal{Z}^{\mp}_{n; \lambda,\bm{h}}}{\mathcal{Z}^{+}_{n; \lambda,\bm{h}}} \right] - \frac{1}{2|\mathcal{W}_n|}\ln\left[ \frac{Q^{+}_{\Delta_n; \bm{\rmh}}}{Q^{-}_{\Delta_n; \bm{\rmh}}} \right].
 \end{equation}

For the second term we use the same bound (\ref{bound.on,Q+/Q-}). When $\h=0$ we get
\begin{equation*}
    \tau_w(J,\lambda,0)=  \lim_{n \to \infty} -\frac{1}{|\mathcal{W}_n|}\ln\left[ \frac{\mathcal{Z}^{\mp}_{n; \lambda, 0}}{\mathcal{Z}^{+}_{n; \lambda,0}} \right].
\end{equation*}
 
 Doing the same bounds as in (\ref{bound.in.Q+}) and (\ref{bound.in.Q-}) we get
 \begin{equation}\label{bound,Z.mp}
     \mathcal{Z}^{\mp}_{n; \lambda,\bm{h}} \leq \exp{ \{ (2n+1)^{d-1}\sum_{k=0}^{\lfloor\frac{n^\alpha}{2}\rfloor} \mid \mathrm{h}_k \mid  \} }\mathcal{Z}^{\mp}_{n; \lambda, 0}
 \end{equation}
 and 
 \begin{equation}\label{bound.Z.+}
      \mathcal{Z}^{+}_{n; \lambda,\bm{h}} \geq - \exp{ \{ (2n+1)^{d-1}\sum_{k=0}^{\lfloor\frac{n^\alpha}{2}\rfloor} \mid \mathrm{h}_k \mid  \} }\mathcal{Z}^{\mp}_{n; \lambda, 0}
 \end{equation}
 that gives us 
 \begin{equation*}
     -\frac{1}{|\mathcal{W}_n|}\ln\left[ \frac{\mathcal{Z}^{\mp}_{n; \lambda, \h}}{\mathcal{Z}^{+}_{n; \lambda,\h}} \right] \geq -\frac{1}{|\mathcal{W}_n|}\ln\left[ \frac{\mathcal{Z}^{\mp}_{n; \lambda, 0}}{\mathcal{Z}^{+}_{n; \lambda,0}} \right] -\frac{2(2n+1)^{d-1}}{|\mathcal{W}_n|} \sum_{k=0}^{\lfloor\frac{n^\alpha}{2}\rfloor} \mid \mathrm{h}_k \mid 
 \end{equation*}
 As before, we can do the opposite bounds on (\ref{bound,Z.mp}) and (\ref{bound.Z.+}) getting 
 
 \begin{equation}
     \mid \frac{1}{|\mathcal{W}_n|}\ln\left[ \frac{\mathcal{Z}^{\mp}_{n; \lambda, \h}}{\mathcal{Z}^{+}_{n; \lambda,\h}} \right] -  \frac{1}{|\mathcal{W}_n|}\ln\left[ \frac{\mathcal{Z}^{\mp}_{n; \lambda, 0}}{\mathcal{Z}^{+}_{n; \lambda,0}} \right] \mid \leq \frac{(2n+1)^{d-1}}{|\mathcal{W}_n|} \sum_{k=0}^{\lfloor\frac{n^\alpha}{2}\rfloor} \mid \mathrm{h}_k \mid.
 \end{equation}
 
 This together with (\ref{bound.on,Q+/Q-}) proves the lemma, just by taking the limit.
 
\end{proof}

\begin{comment}

To finish this section, we put together Proposition \ref{compare.st.and.integral} and  Lemma \ref{compare.surface.tension} and reintroduce $\beta$ to understand the dependence of the temperature on the phase transition. Doing so, we conclude

\begin{equation*}
 \tau_w(\beta J,\beta\lambda, 0)  - 6\beta\sum_{k=0}^\infty \mid \mathrm{h}_k \mid \leq \int_0^{\beta\lambda} \langle\sigma_0 \rangle^{+, \bm{\rmh}}_{J,s} - \langle \sigma_0 \rangle^{-,\bm{h}}_{J,s} ds.
\end{equation*}

\end{comment}
